DPN-SENet:A self-attention mechanism neural network for detection and diagnosis of COVID-19 from chest x-ray images

Background and Objective: The new type of coronavirus is also called COVID-19. It began to spread at the end of 2019 and has now spread across the world. Until October 2020, It has infected around 37 million people and claimed about 1 million lives. We propose a deep learning model that can help radiologists and clinicians use chest X-rays to diagnose COVID-19 cases and show the diagnostic features of pneumonia. Methods: The approach in this study is: 1) we propose a data enhancement method to increase the diversity of the data set, thereby improving the generalization performance of the model. 2) Our deep convolution neural network model DPN-SE adds a self-attention mechanism to the DPN network. The addition of a self-attention mechanism has greatly improved the performance of the network. 3) Use the Lime interpretable library to mark the feature regions on the X-ray medical image that helps doctors more quickly diagnose COVID-19 in people. Results: Under the same network model, the data with and without data enhancement is put into the model for training respectively. At last, comparing two experimental results: among the 10 network models with different structures, 7 network models have improved their effects after using data enhancement, with an average improvement of 1% in recognition accuracy. We propose that the accuracy and recall rates of the DPN-SE network are 93% and 98% of cases (COVID vs. pneumonia bacteria vs. viral pneumonia vs. normal). Compared with the original DPN, the respective accuracy is improved by 2%. Conclusion: The data augmentation method we used has achieved effective results on a small amount of data set, showing that a reasonable data augmentation method can improve the recognition accuracy without changing the sample size and model structure. Overall, the proposed method and model can effectively become a very useful tool for clinical radiologists.

==> append.tex <==

%
\section*{Appendix}




%

\section{Class-agnostic Precision-recall Curves}
\begin{table}[!h]
\centering 
\small
\begin{tabular}{ l| c | c c c }
Method & AP & AP$_{50}$ & AP$_{75}$ & AP$_{90}$ \\
\Xhline{2\arrayrulewidth}
Orginal RetinaNet \cite{lin2017focal} & 39.5 & 63.6 & 41.8 & 10.6 \\
RetinaNet w/ GN \cite{wu2018group} & 40.0 & 64.5 & 42.2 & 10.4 \\
\Ours & \textbf{40.5} & \textbf{64.7}  & \textbf{42.6} & \textbf{13.1} \\
\hline
& & +0.2 & +0.4 & +2.7
\end{tabular}
\vspace{0.2cm}
\caption{The class-agnostic detection performance for RetinaNet and \Ours. \Ours\ has better performance than RetinaNet. Moreover, the improvement over RetinaNet becomes larger with a stricter IOU threshold. The results are obtained with the same models in Table 4 of our main paper.}
\label{table:detection_performance}
\end{table}

In Fig.~\ref{fig:pr_iou_50}, Fig.~\ref{fig:pr_iou_75} and Fig.~\ref{fig:pr_iou_90}, we present class-agnostic precision-recall curves on split $\tt minival$
at IOU thresholds being 0.50, 0.75 and 0.90, respectively. Table \ref{table:detection_performance} shows APs corresponding to the three curves.

As shown in Table \ref{table:detection_performance}, our \Ours\ achieves better performance than its anchor-based counterpart RetinaNet. Moreover, it worth noting that with a stricter IOU threshold, \Ours\ enjoys a larger improvement over RetinaNet, which suggests that \Ours\ has a better bounding box regressor to detect objects more accurately. One of the reasons should be that \Ours\ has the ability to leverage more foreground samples to train the regressor as mentioned in our main paper.

Finally, as shown in all precision-recall curves, the best recalls of these detectors in the precision-recall curves are much lower than $90\%$. It further suggests that the small gap ($98.40\%$ vs. $99.23\%$) of \textit{best possible recall (BPR)} between \Ours\ and RetinaNet hardly harms the final detection performance.

\begin{figure}[t!]
\begin{center}
\includegraphics[width=\linewidth]{latex/figures/pr_iou_at_50.pdf}
\end{center}
   \caption{Class-agnostic precision-recall curves at IOU $= 0.50$.}
\label{fig:pr_iou_50}
\end{figure}

\begin{figure}[t!]
\begin{center}
\includegraphics[width=\linewidth]{latex/figures/pr_iou_at_75.pdf}
\end{center}
   \caption{Class-agnostic precision-recall curves at IOU $= 0.75$.}
\label{fig:pr_iou_75}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=\linewidth]{latex/figures/pr_iou_at_90.pdf}
\end{center}
   \caption{Class-agnostic precision-recall curves at IOU $= 0.90$.}
\label{fig:pr_iou_90}
\end{figure}



\section{Visualization for Center-ness}
\begin{figure*}[t!]
\begin{center}
    \includegraphics[width=.8\linewidth]{latex/figures/centerness-append.pdf}
\end{center}
   \caption{Without (left) or with (right) the proposed center-ness. A point in the figure denotes a detected bounding box. The dashed line is the line $y = x$. As shown in the figure (right), after multiplying the classification scores with the center-ness scores, the low-quality boxes (under the line $y=x$) are pushed to the left side of the plot. It suggests that the scores of these boxes are reduced substantially.}
\label{fig:centerness}
\end{figure*}
As mentioned in our main paper, by suppressing low-quality detected bounding boxes, the proposed center-ness branch improves the detection performance by a large margin. In this section, we confirm this. 
%

We expect that the center-ness can down-weight the scores of low-quality bounding boxes such that these bounding boxes can be filtered out in following post-processing such as non-maximum suppression (NMS). A detected bounding box is considered as a low-quality one if it has a low IOU score with its corresponding ground-truth bounding box. 
A bounding box with low IOU but  a high confidence score  is likely to become a false positive and harm the precision.

In Fig.~\ref{fig:centerness}, we consider a detected bounding box as a 2D point $(x, y)$ with $x$ being its score and $y$ being the IOU with its corresponding ground-truth box. As shown in Fig.~\ref{fig:centerness} (left), before applying the center-ness, there are a large number of low-quality bounding boxes but with a high confidence score (i.e., the points under the line $y=x$). Due to their high scores, these low-quality bounding boxes cannot be eliminated in post-processing and result in 
%
lowering the precision of the detector.
%
%
After multiplying the classification score with the center-ness score, these points are pushed to %
the left side of the plot
(i.e., their scores are reduced), as shown in Fig.~\ref{fig:centerness} (right). As a result, these low-quality bounding boxes are much more likely to be filtered out in post-processing and the final detection performance can be improved.
%


\section{Qualitative Results}
\begin{figure*}
\begin{center}
\includegraphics[width=\linewidth]{latex/figures/results.pdf}
\end{center}
   \caption{Some detection results on $\tt minival$ split. ResNet-50 is used as the backbone. As shown in the figure, \Ours\ works well with a wide range of objects including crowded, occluded, highly overlapped, extremely small and very large objects.}
\label{fig:visualization_results}
\end{figure*}
Some qualitative results are shown in Fig. \ref{fig:visualization_results}. As shown in the figure, our proposed \Ours\ can detect a wide range of objects including crowded, occluded, highly overlapped, extremely small and very large objects.








==> rebuttal.tex <==

\def\Ours{{FCOS}\xspace}
\def\eg{{\it e.g.}\xspace}
\def\ie{{\it i.e.}\xspace}




%%%%%%%%% BODY TEXT - ENTER YOUR RESPONSE BELOW
\section{More discussions}
\noindent\textbf{Center-ness vs.\ IoUNet:}


 Center-ness and IoUNet of Jiang et al.\ ``Acquisition of Localization Confidence for Accurate Object Detection''
  shares a similar purpose (\ie, to suppress low-quality predictions) with different approaches.
  IoUNet trains a separate network to predict the IoU score between predicted bounding-boxes and ground-truth boxes. Center-ness, as a part of our
   detector, only has a single layer and is trained jointly with the detector, thus being much simpler. Moreover, ``center-ness'' does not take as input the predicted bounding-boxes. Instead, it directly accesses the location's ability to predict high-quality bounding-boxes.

\noindent\textbf{BPR in Section 4.1 and ambiguity analysis:}

%\begin{itemize}
%    \itemsep -0.2cm
%\item We confirm that each sample is used at most once.
%\item
 We do not aim to compare ``recall by specific IoU" with ``recall by pixel within box".
 The main purpose of Table 1 is to show that the upper bound of recall of \Ours is very close to the upper bound of recall of anchor-based RetinaNet (98.4\%  vs.\ 99.23\%).
 BPR by other IoU thresholds are listed as those
  are used in the official code of RetinaNet. Moreover, \textit{no evidence shows that the regression targets of \Ours are difficult to learn because they are more spread-out.}  \Ours in fact yields more accurate bounding-boxes.
%\item



 During training, we deal with the ambiguity at the same FPN level by choosing the ground-truth
  box with the minimal area. When testing, if two objects A and B with the same class have overlap,
  no matter which one object the locations in the overlap predict, the prediction is correct and the missed one can be predicted by the locations only belonging to it. In the case that A and B do not belong to the same class,
  a location in the overlap might predict A's class but regress B's bounding-box, which is a mistake.
  That is why we only count the ambiguity across different classes. Moreover,
it appears that
  {this ambiguity does not make \Ours worse than RetinaNet in AP, as shown in Table \ref{table:ablation_study}.}

%\end{itemize}




\noindent\textbf{Additional ablation study:}

\noindent
 As shown in Table \ref{table:ablation_study}, a  vanilla
  \Ours performs on par with RetinaNet, being of
   simpler design and with $\sim9\times$ less network outputs. Moreover, \Ours works much better than RetinaNet with single anchor.
   %More comparisons with single anchor (as suggested by R3) will be added.
   As for the $2\%$ gain on $\tt test$-$\tt dev$, besides the performance gain brought by the components in Table \ref{table:ablation_study}, we conjecture that different training details (\eg, learning rate schedule) might
% bring the remaining performance gain.
cause slight differences in performance.
%We have made our best to make the comparison as
%fair as possible.
%However, official RetinaNet codes [6] do not include the training details of the models evaluated on $\tt test$-$\tt dev$ and thus it is difficult.
%to make an absolutely fair comparison.
%Our released codes will include all training details of the models evaluated on \texttt{test-dev}.
%Finally, we do not view group normalization, scalars, $P_5$ and IoU Loss as ``bells and whistles" because they can be implemented in a few lines of codes and almost cost-free when testing.
%However, we will remove the claim to avoid the ambiguity.
%Importantly, \textit{Table \ref{table:ablation_study} shows
%that FCOS works well even without these small design choices.}


\begin{table}[t!]
\centering
\small
\begin{tabular}{l | c c c c | c}
Method & $C_5/P_5$ & GN & Scalar & IoU & AP \\
\Xhline{2\arrayrulewidth}
RetinaNet (\#A=1) & $C_5$ & & & & 32.5 \\
RetinaNet (\#A=9) & $C_5$ & & & & 35.7 \\
\hline
% \Ours w/o ctr & $C_5$ & & & & 32.6 \\
\Ours (pure) & $C_5$ & & & & 35.7 \\
\Ours & $P_5$ & & & & 35.8 \\
\Ours & $P_5$ & \checkmark & & & 36.3 \\
\Ours & $P_5$ & \checkmark & \checkmark & & 36.4 \\
\Ours & $P_5$ & \checkmark & \checkmark & \checkmark & \textbf{36.6} \\
\end{tabular}
\caption{Ablation study on MS-COCO \texttt{minival}. ``\#A" is the number of anchor boxes per location in RetinaNet. ``IOU" is IOU loss. ``Scalar" denotes whether to use scalars in $\exp$. All experiments are conducted with the same settings.}
\label{table:ablation_study}
\end{table}

\noindent\textbf{RetinaNet with Center-ness: %or scalars:
}

%\noindent
 Center-ness cannot be directly used in RetinaNet with multiple anchor boxes per location because one location on feature maps has \textit{only one} center-ness score but different anchor boxes on the same location require different ``center-ness"
 (note that center-ness is also used as ``soft" thresholds for positive/negative samples).

  For anchor-based RetinaNet, the IoU score between anchor boxes and ground-truth boxes may serve as an alternative of ``center-ness".
  % and we will add the experiments in the revised version, but in fact this is beyond the focus of this paper that focuses on the much simpler anchor-free setting. As for scalars, scalars only improve the performance by $0.1\%$ (Table \ref{table:ablation_study}). Moreover, RetinaNet \textit{normalizes} its regression training targets by the anchor boxes of each FPN level, which further makes scalars useless in RetinaNet.

%\noindent\textbf{ \Ours at high IoU thresholds:}

%\noindent Yes,
%\Ours works well at high IoU thresholds, for example FCOS 32.9\% vs.\ RetinaNet 31.5\% in AP$_{80}$.
%But scalar variables only help this a little. \Ours without scalar variables achieves almost the same performance (32.8\% in AP$_{80}$). IOU loss and more foreground locations used to train the regressor also help it. Analyses will be added when revising.

\noindent\textbf{Positive samples overlap with RetinaNet:}

%\noindent
 We want to highlight that center-ness comes into play \textit{only} when testing. When training, all locations within ground-truth
  boxes are marked as positive samples. As a result, \Ours can use more foreground locations to train the regressor and thus yield more accurate bounding-boxes.


